Polylogarithmic Sketches for Clustering

Given $n$ points in $\ell_p^d$, we consider the problem of partitioning points into $k$ clusters with associated centers. The cost of a clustering is the sum of $p^{\text{th}}$ powers of distances of points to their cluster centers. For $p \in [1,2]$, we design sketches of size poly$(\log(nd),k,1/\epsilon)$ such that the cost of the optimal clustering can be estimated to within factor $1+\epsilon$, despite the fact that the compressed representation does not contain enough information to recover the cluster centers or the partition into clusters. This leads to a streaming algorithm for estimating the clustering cost with space poly$(\log(nd),k,1/\epsilon)$. We also obtain a distributed memory algorithm, where the $n$ points are arbitrarily partitioned amongst $m$ machines, each of which sends information to a central party who then computes an approximation of the clustering cost. Prior to this work, no such streaming or distributed-memory algorithm was known with sublinear dependence on $d$ for $p \in [1,2)$.

==> Sketching.tex <==
%!TEX root = MST.tex


\subsection{Useful Facts}

We begin with some useful facts. We first define stable random variables.
\begin{definition}\label{def:stable}
	A distribution $\mathcal{D}$ is said to be $p$-stable if whenever $X_1,\dots,X_n \sim \mathcal{D}$ are drawn independently and $a \in \R^n$ is a fixed vector, we have
	\[	\sum_{i=1}^n a_i X_i = \|a\|_p X	\]
	where $X \sim \mathcal{D}$ is again drawn from the same distribution, and the ``$=$'' symbol above denotes distributional equality. For $p \in (0,2]$, we define the \textit{standard $p$-stable distribution}, denoted $\cD_p$, to be the distribution with characteristic function 
	\[\exx{Z \sim \cD_p}{e^{itZ}	} = e^{-|t|^p}\]
	which is, in fact, is $p$-stable. %In particular, for $p=2$, the standard $2$-stable distribution $\cD_2$ is just the normal distribution $\mathcal{N}(0,1)$ (i.e., $\sum_i a_i g_i = g \cdot \|a\|_2$, where $g,g_1,\dots,g_n$ are Gaussian), and the standard $1$-stable distribution $\cD_1$ is the \textit{Cauchy Distribution}.
\end{definition}
Standard methods for generating $p$-stable random variables are discussed in \cite{nolan2009stable}.
%Note for $p<2$, the distributions have heavy tails -- namely we have the following fact.
%\begin{fact}[Chapter 1.5 \cite{nolan2009stable}]\label{fact:pstabletail}
%	Fix $p \in (0,2)$, and let $\cD_p$ be the standard $p$-stable distribution. Then there is a constant $C_p$ depending only on $p$, such that for any $t >0$, we have
%	\[	\lim_{t \to \infty } \frac{\prb{X \sim \cD_p}{|X| > t}}{C_p \frac{1}{t^p}}= 1	\]
%\end{fact}



\begin{proposition}[\cite{chambers1976method}]\label{prop:genstable}
	Fix any $p \in (0,1)$. Then $X \sim \cD_p$ can be generated as follows:
	\begin{enumerate}
		\item Generate $\theta \sim \text{Uniform}[-\frac{\pi}{2},\frac{\pi}{2}]$.
		\item Generate $r \sim \text{Uniform}[0,1]$.
		\item Set 
		\[X \leftarrow \frac{\sin(p \theta)}{\cos^{1/p}(\theta)} \cdot \left(\frac{\cos(\theta(1-p))}{\ln(1/r)}\right)^{\frac{1-p}{p}}\]
	\end{enumerate}
	\end{proposition}

By Proposition \ref{prop:genstable}, it follows that if we want to generate $X \sim |\cD_p|$, we can generate $\theta \sim \text{Uniform}[-\frac{\pi}{2},\frac{\pi}{2}]$ and $r \sim \text{Uniform}[0,1]$, and set 

\begin{align*}
X &= \left|  \frac{\sin(p \theta)}{\cos^{1/p}(\theta)} \cdot \left(\frac{\cos(\theta(1-p))}{\ln(1/r)}\right)^{\frac{1-p}{p}}\right| \\
&= \frac{|\sin(p \theta)|}{\cos^{1/p}(\theta)} \cdot \left(\frac{\cos(\theta(1-p))}{\ln(1/r)}\right)^{\frac{1-p}{p}}\\
\end{align*}
Notice that since $\cos(\theta(1-p))$ is symmetric around the origin in $\theta$, the entire function above is symmetric around the origin in $\theta$. Thus, we have the following corollary.

\begin{corollary}\label{cor:genstable}
	Fix any $p \in (0,1)$. Then $X \sim |\cD_p|$ can be generated as follows:
	\begin{enumerate}
		\item Generate $\theta \sim \text{Uniform}[0,\frac{\pi}{2}]$.
		\item Generate $r \sim \text{Uniform}[0,1]$.
		\item Set 
		\[X \leftarrow \frac{\sin(p \theta)}{\cos^{1/p}(\theta)} \cdot \left(\frac{\cos(\theta(1-p))}{\ln(1/r)}\right)^{\frac{1-p}{p}}\]
	\end{enumerate}
\end{corollary}


In what follows, we define a function function $g(r,\theta): (0,1) \times (0,\pi/2) \to \R$ via
\[g(r,\theta) = \frac{\sin(p \theta)}{\cos^{1/p}(\theta)} \cdot \left(\frac{\cos(\theta(1-p))}{\ln(1/r)}\right)^{\frac{1-p}{p}}\]

We now prove some facts about $g(r,\theta)$

\begin{proposition}\label{prop:monotoneg}
	Define the function $g(r,\theta)$ as above, with the domain $(0,1) \times (0,\frac{\pi}{2})$. Then $g$ is monotone increasing in both parameters.
	\end{proposition}
\begin{proof}
First, fix any $\theta \in (0,\pi/2)$. Then since $\ln(1/r)$ is decreasing as $r$ increases in $(0,1)$ the value $(\frac{1}{\ln(1/r)})^{(1-p)/p}$ is monotone decreasing in $r$, as needed. For the second part, notice that $\sin(p \theta)$ is monotone increasing in $\theta$. Thus, it suffices to show that the function

\[	\frac{\cos(\theta(1-p))^{1-p}}{\cos(\theta)}	\]
is monotone increasing.  We have

\[\frac{\partial}{\partial \theta} \frac{\cos ^{1-p}(\theta (1-p))}{\cos (\theta )}=\tan (\theta ) \sec (\theta ) \cos ^{1-p}(\theta (1-p))\]

Note that all three of $\tan (\theta ), \sec (\theta ) ,$ and $\cos(\theta(1-p))$ are positive for $\theta \in (0,\pi/2)$, which completes the claim and the proof of the Proposition
\end{proof}

We obtain the following corollary.

\begin{corollary}
	Define the function $g(r,\theta)$ as above, with the domain $(0,1) \times (0,\frac{\pi}{2})$. Then we have
	\[|\median(\cD_p)| = g\left(\frac{1}{2},\frac{\pi}{4}\right)	\]
	Where $|\median(\cD_p)|$ is the value such that
	\[			\prb{X \sim \cD_p}{|X| < |\median(\cD_p)|} =1/2	\]
	\end{corollary}


\begin{lemma}\label{lemma:stablemedianbound}
	Fix any $p \in (0,1)$ and $\eps >0$, and let $R =|\median(\cD_p)|$.  Then there exists a constant $C$ independent of $p,\eps$ such that
	
	\[	\prb{X \sim \cD_p}{R \leq |X| \leq (1+  \eps)R} \geq C p^2 \eps^2  \]
	and 
		\[	\prb{X \sim \cD_p}{(1-\eps)R \leq |X| \leq R} \geq C p^2 \eps^2  \]
\end{lemma}
\begin{proof}
	Define the function $g(r,\theta)$ as above, and recall by Corollary \ref{cor:genstable} that we can generate $X \sim |\cD_p|$ by picking $r \sim [0,1],\theta \sim [0,\pi/2]$ and setting $X = g(r,\theta)$. Moreover, we know by the prior discussion that $R = g(1/2,\pi/4)$. We will proceed by bounding the partial derivatives of $\ln(g(r,\theta))$ by a value $\Omega(1/p)$ for any $r,\theta$ bounded away from the edges of the domain box $(0,1) \times (0,\pi/2)$. We have
	
	
	\[\frac{\partial}{\partial \theta}	\ln(g(r,\theta))  = \frac{\cos(p \theta)}{\sin (p \theta)} - \frac{(1-p)^2}{p} \frac{\sin(\theta(1-p))}{\cos(\theta(1-p))} + \frac{1}{p} \frac{\sin(\theta)}{\cos(\theta)}	\]
	
	For $\theta$ in the interval $(1/100,\pi/2 - 1/100)$, the above derivative is bounded in magnitude by $C_1 p^{-1}$, for some constant $C_1$. For the second partial derivative, we have
		\[\frac{\partial}{\partial r}	\ln(g(r,\theta)) =\frac{\partial}{\partial r} -(1-p)/p \ln(\ln(1/r))= \frac{1-p}{p}  \frac{1}{r \log(1/r)}  \]
	Again, for $r$ in the interval $[1/100,99/100]$, the above is bounded by $C_1 p^{-1}$. It follows that if $I_1 \times I_2$ is the product of any two intervals inside with $I_1 \subset (\frac{1}{100},\frac{99}{100}) $ and $I_2 \subset  (1/100,\pi/2-1/100)$ Then we have
	
	\[	\max_{(r_1,\theta_1),(r_2,\theta_2) \in I_1 \times I_2} \left|\ln(g(r_1,\theta_1)) - \ln(g(r_2,\theta_2)) \right| \leq \frac{C_1( |I_1| + |I_2|)}{p}	\]
	
It follows that for intervals $I_1,I_2$ with $|I_1| - |I_2| < c \eps  p $ for a sufficiently small constant $c$, it follows that 
	
		\[	\max_{(r_1,\theta_1),(r_2,\theta_2) \in I_1 \times I_2} \left|\frac{g(r_1,\theta_1)}{ g(r_2,\theta_2)} \right| \leq \exp\left(\frac{C_1( |I_1| + |I_2|)}{p} \right) \leq 1+ \eps	\]
	We apply the above fact with $I_1 = [1/2 - \gamma, 1/2 + \gamma]$ and $I_2 = (\pi/4 - \gamma, \pi/4 + \gamma)$, where $\gamma = c p \eps /4$. Let $I_1^+ = [1/2,1/2+ \gamma], I_1^- = [1/2 - \gamma, 1/2]$ and $I_2^+ =[\pi/4 , \pi/4 + \gamma$ and $I_2^- = [\pi/4 - \gamma, \pi/4]$. By the monotonicty of $g$ (Proposition \ref{prop:monotoneg}), and the above paragraphs, it follows that 
	$$R \leq g(r,\theta) \leq (1+\eps)R$$
	For all $(r,\theta) \in I_1^+ \times I_2^+$, and moreover 
	$$(1-\eps)R \leq g(r,\theta) \leq R$$
	For all $(r,\theta) \in I_1^- \times I_2^-$.
	Moreover, the area of both $I_1^+ \times I_2^+$ and $I_1^- \times I_2^-$ is $\Omega(p^2 \eps^2)$, from which it follows that the probability that $(r,\theta)$ is in $I_1^+ \times I_2^+$ is at least $\Omega(p^2 \eps^2)$, and similarly for $I_1^- \times I_2^-$, which completes the proof of the Lemma.

 


\end{proof}


We are now ready to prove the correctness of the Indyk $p$-stable sketch. 
\begin{theorem}[Indyk's $p$-Stable Sketch]\label{thm:indykPrelims}
Fix $1/2 > p > 0$ and $\eps \in (0,1)$, and set $t = \Theta(\frac{1}{(p\eps)^4} \log\delta^{-1})$ Let $\bX_1,\dots,\bX_t \sim \cD_p$ independently. Then, with probability $1-\delta$, we have
\[1-\eps\leq	\median_{i \in [t]} \left\{	\frac{|\bX_i|}{|\median(\cD_p)|}	\right\}  \leq 1+\eps		\]
Where $|\median(\cD_p)|$ is the value such that
\[			\prb{X \sim \cD_p}{|X| < |\median(\cD_p)|} =1/2	\]
\end{theorem}
\begin{proof}
	Set $R = |\median(\cD_p)|$. By Lemma \ref{lemma:stablemedianbound}, we have both $	\prb{X \sim \cD_p}{r \leq |X| \leq (1+\eps)r} = \Omega(p^2 \eps^2)$, and $\prb{X \sim \cD_p}{(1-\eps)r \leq |X| \leq r} = \Omega(p^2\eps^2)$. It follows that  there exists a constant $c>0$ such that for each trial $\bX_i$, the probability that $\bX_i > (1+\eps )R$ is at most $1/2 - c p^2 \eps^2$, and the probability that $\bX_i < (1-\eps)R$ is at most $1/2 - c p^2 \eps^2$.	
	 By Chernoff bounds, we have
	
	\[	\pr{ \left|	\left\{ i \in [t] \; | \; \bX_i > (1+\eps)R	\right\}	\right| \geq 1/2} < e^{- \eps^4 p^4  t/3} 	\]
	and 
			\[	\pr{ \left|	\left\{ i \in [t] \; | \; \bX_i < (1-\eps)R	\right\}	\right| \geq 1/2} < e^{- \eps^4 p^4  t/3} 	\]
	Conditioned on both of these events occurring simultaneously, which occurs with probability at least $1- 2 e^{- \eps^4 p^4  t/3} > 1-\delta$, the median must fall within the range $(1-\eps)R$ and $(1+\eps)R$. Thus, we have:
			\[	\pr{	\median_{i \in [t]} \left\{	\frac{|\bX_i|}{|\median(\cD_p)|} \right\}= (1\pm\eps) r} > 1-\delta	\]
		as needed.
			

\end{proof}
